Skein theory for the D_{2n} planar algebras

We give a combinatorial description of the ``$D_{2n}$ planar algebra,'' by generators and relations. We explain how the generator interacts with the Temperley-Lieb braiding. This shows the previously known braiding on the even part extends to a `braiding up to sign' on the entire planar algebra. We give a direct proof that our relations are consistent (using this `braiding up to sign'), give a complete description of the associated tensor category and principal graph, and show that the planar algebra is positive definite. These facts allow us to identify our combinatorial construction with the standard invariant of the subfactor $D_{2n}$.

==> documentclasshack.tex <==
%auto-ignore
%%%%%% a hack to make the documentclass name available later %%%
% Thanks to Morten Høgholm. I stole this code from 
% http://groups.google.com/group/comp.text.tex/msg/142306cc7f8acdac
\let\LaTeXdocumentclass\documentclass
\renewcommand*\documentclass[2][]{%
   \newcommand*\ClassName{#2}% for later use
   \LaTeXdocumentclass[#1]{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> todolist.tex <==
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.
\section*{todo list}
Priorities:
\begin{itemize}
\item[Noah] Decide what references to use for generators and relations
for BMW/Hecke.
\item[Noah] Write a paragraph about other constructions of $D_{2n}$.
Mueger: \cite{MR1749250}, Feng: \cite{MR1867572}.
\item[Emily]  Think about table of contents
\end{itemize}

\begin{enumerate}
\item Add irreducibility to the main theorem?
\item Describe the inclusion of $A_{4n-3}$ into $D_{2n}$, and what
this does to projections.
\hrule%
\end{enumerate}


==> xypdf-c.tex <==
%% xypdf-c.tex from $Id: xypdf-c.doc,v $
%%
%% Xy-pic ``Colour extension'' PDF backend support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-cloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-cloaded\endcsname=\empty \xycatcodes
\expandafter\ifx \csname xypdf-sloaded\endcsname\empty\else
 \xyinputorelse@{xypdf-s}{\xyerror@{Could not load xypdf-s}{}}%
 \xycatcodes\fi
\xydef@\UsePDFcolor{\installPDFcolor@}
\xydef@\NoPDFcolor{\UnloadColor@}
\xydef@\installPDFcolor@{\installPDFstyle@
 \let\xymath@=\xyPDFmath@ \let\xynomath@=\xyPDFnomath@
 \let\checkxyPDFcolor@=\checkxyPDFcolor@@
 \let\xycolor@@=\xyPDFcolor@@
 \xystandardcolors@ 
 \xyuncatcodes }
\xydef@\xyPDFmath@{\hbox\bgroup\dimen@=.55ex \checkxyPDFcolor@ \xyinside@}
\xydef@\xyPDFnomath@{\hbox\bgroup\dimen@=\z@ \checkxyPDFcolor@ \xyinside@}
\xydef@\checkxyPDFcolor@@{\edef\pdfsaved@color{\pdfcurrent@color}%
 \let\checkxyPDFcolor@=\relax}
\xylet@\checkxyPDFcolor@=\relax
\xydef@\xyPDFnewcolor@#1#2#3#4#5{%
 \expandafter\DN@\expandafter{\csname shape [#1]\endcsname}%
 \DNii@{\relax}\ifx\next@\nextii@\newxycolor{#1}{}\relax\fi
 \DNii@{#4}\ifx\nextii@\empty
 \expandafter\DNii@\expandafter{\csname xyPDFshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPDFcolor@{#2//#3}}\else
 \expandafter\DNii@\expandafter{\csname xyPDFshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPDFcolor@{#4}}\fi
 \ifx\nextii@\empty\expandafter\def\next@{\xyPDFnotimplemented@@`#1'@@}%
 \else
 \edef\tmp@{\noexpand\let\expandafter\noexpand\next@
 \expandafter\noexpand\nextii@}\expandafter\tmp@\fi }
\xylet@\newxycolor@=\xyPDFnewcolor@
\xydef@\xyPDFcolor@{\ifPDFspecials@\expandafter\xyPDFcolor@@
 \else\expandafter\eat@\fi}
\xydef@\xyPDFcolor@@#1{\bgroup \checkXyStyle@ 
 \def\preStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPDFpre@}}%
 \def\postStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPDFpost@}}%
 \let\modPDFboxz@=\modXYstyle@ \xyPDF@color@@{#1}%
 \toks@={\egroup\let\xy@style@=\relax \def\Drop@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Drop@@}\def\Connect@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Connect@@}}%
 \the\toks@ }

\xydef@\pdfcurrent@color{1 1 1 1 k 1 1 1 1 K}
\xydef@\pdfsaved@color{1 1 1 1 k 1 1 1 1 K}
\xydef@\xyPDF@color@@#1{%
 \edef\pdfsaved@color{\pdfcurrent@color}%
 \pdf@convertcolor#1////!%
 \edef\next@{\noexpand\xyPDFsplitPDF@{\pdfcurrent@color}{\pdfsaved@color}}%
 \next@}
\xydef@\pdf@convertcolor#1//#2//#3!{\DN@{#2}%
 \DNii@{cmyk}\ifx\next@\nextii@\DN@{#1 k #1 K}%
 \else \DNii@{rgb}\ifx\next@\nextii@\DN@{#1 rg #1 RG}%
 \else \DNii@{gray}\ifx\next@\nextii@\DN@{#1 #1 #1 rg #1 #1 #1 RG}%
 \else \DN@{1 1 1 1 k 1 1 1 1 K}%
 \fi \fi \fi 
 \expandafter\def\expandafter\pdfcurrent@color\expandafter{\next@}}
\xydef@\xycolor@raw@@#1{}%
\endinput


==> xypdf-f.tex <==
%% xypdf-f.tex from $Id: xypdf-f.doc,v $
%%
%% Xy-pic ``Frame extension'' PDF backend support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-floaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-floaded\endcsname=\empty \xycatcodes
\xydef@\installPDFframes@{%
 \let\framed@body@@=\xyPDFframed@body@
 \let\circled@x@@=\xyPDFcircled@x@
 \let\ellipsed@x@@=\xyPDFellipsed@x@
 \installPDFfills@
 \xyuncatcodes}
\xydef@\UsePDFframes{\installPDFframes@}
\xydef@\NoPDFframes{\UnloadFrames@}
\xydef@\xyPDFframed@body@{\DN@{\framed@body@}%
 \ifx\framehfill\frm@solidh@@
 \DN@{\xyPDFframed@oval@\xyPDFoval@Special}%
 \else\ifdim\R@=\z@\else
 \ifx\framehfill\frm@dashh@@
 \DN@{\xyPDFframed@oval@\xyPDFdashoval@Special}%
 \else\ifx\framehfill\frm@doth@@
 \DN@{\xyPDFframed@oval@\xyPDFdotoval@Special}%
 \fi\fi
 \fi\fi \next@ }
\xydef@\xyPDFframed@oval@#1{\vglue\U@c
 \hbox{\hglue\L@c\xypdfoval@#1\hglue\R@c}\vglue\D@c}
\xydef@\xyPDFcircled@x@{\DN@{\xyPDFcircled@x@@\xyPDFcirc@Special}%
 \ifx\framehfill\frm@doth@@
 \DN@{\xyPDFcircled@x@@\xyPDFdotcirc@Special}%
 \else\ifx\framehfill\frm@dashh@@
 \DN@{\xyPDFcircled@x@@\xyPDFdashcirc@Special}%
 \fi\fi \next@ }
\xydef@\xyPDFcircled@x@@#1{\vglue2\R@
 \hbox{\hglue2\R@\xypdfcircle@#1\hglue2\R@}%
 \vglue2\R@}
\xydef@\xyPDFellipsed@x@#1#2{%
 \DN@{\xyPDFellipsed@x@@\xyPDFcirc@Special}%
 \ifx\framehfill\frm@doth@@
 \DN@{\xyPDFellipsed@x@@\xyPDFdotcirc@Special}%
 \else\ifx\framehfill\frm@dashh@@
 \DN@{\xyPDFellipsed@x@@\xyPDFdashcirc@Special}%
 \fi\fi \next@{#1}{#2}}
\xydef@\xyPDFellipsed@x@@#1#2#3{\vglue #3\vglue #3\relax
 \hbox{\L@c = #2\relax \R@c=\L@c \D@c = #3\relax \U@c=\D@c 
 \hglue#2\hglue#2\relax\xypdfellipse@#1\hglue#2\hglue#2\relax}%
 \vglue #3\vglue #3\relax}
\xydef@\xyPDFdashhfill@{{\SemiDirectionChar=95 \Direction=3072 \xyPDFdash@}}
\xydef@\xyPDFdashvfill@{{\SemiDirection=31 \Direction=1023 \xyPDFdash@}}
\xydef@\xypdfoval@#1{%
 \dimen@=\L@c \advance\dimen@\R@c
 \dimen@ii=\U@c \advance\dimen@ii\D@c 
 \ifdim\dimen@ii<\dimen@ \relax \dimen@=\dimen@ii\fi \divide\dimen@\tw@
 \ifdim\R@>\dimen@ \relax \R@=\dimen@ \fi
 \D@c=-\D@c \L@c=-\L@c 
 \edef\tmp@{\expandafter\removePT@\the\R@
 \space\expandafter\removePT@\the\R@c 
 \space\expandafter\removePT@\the\D@c 
 \space\expandafter\removePT@\the\L@c 
 \space\expandafter\removePT@\the\U@c }%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xypdfcircle@#1{\dimen@=\R@
 \edef\tmp@{\expandafter\removePT@\the\dimen@}%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xypdfellipse@#1{\edef\tmp@{%
 \expandafter\removePT@\the\U@c \space
 \expandafter\removePT@\the\D@c \space
 \expandafter\removePT@\the\L@c \space
 \expandafter\removePT@\the\R@c }%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xyPDFoval@Special#1{\PDFmacro@{#1 ov}}%%%%<<<---- here
\xydef@\xyPDFcirc@Special#1{\PDFmacro@{#1 ox}}%%%%<<<---- here
\xydef@\xyPDFdotcirc@Special#1{\PDFmacro@{#1 ot}}%%%%<<<---- here
\xydef@\xyPDFdashcirc@Special#1{\PDFmacro@{#1 od}}%%%%<<<---- here
\xydef@\xyPDFdotoval@Special#1{\PDFmacro@{#1 vt}}%%%%<<<---- here
\xydef@\xyPDFdashoval@Special#1{\PDFmacro@{#1 vd}}%%%%<<<---- here
\xydef@\xyPDFfilledRegion#1#2{\setboxz@h{\lower\D@c\vbox{%
 \vglue\U@c\hbox{#1#2\empty\hglue\L@c\hglue\R@c}\vglue\D@c}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\filledRectangle@PDF{%
 \xyPDFfilledRegion{\xypdfoval@\xyPDFfilloval@Special}}
\xydef@\filledCircle@PDF#1{{\R@c=\R@ \L@c=\R@ \U@c=\R@ \D@c=\R@
 \xyPDFfilledRegion{\xypdfcircle@\xyPDFfillcirc@Special}#1}}
\xydef@\filledEllipse@PDF{%
 \xyPDFfilledRegion{\xypdfellipse@\xyPDFfillellipse@Special}}
\xydef@\filledOval@PDF{%
 \xyPDFfilledRegion{\xypdfoval@\xyPDFfilloval@Special}}
\xydef@\frame@emph@PDF#1{\filled@{#1}\relax}
\xydef@\installPDFfills@{%
 \let\frame@emph@@=\frame@emph@PDF
 \let\filledRectangle@@=\filledRectangle@PDF
 \let\filledOval@@=\filledOval@PDF
 \let\filledCircle@@=\filledCircle@PDF
 \let\filledEllipse@@=\filledEllipse@PDF
}
\xydef@\xyPDFfilloval@Special#1#2{%
 \ifx#2\relax\PDFmacro@{#1 sfo}%%%%%<<<---- here
 \else\PDFmacro@{#1 fo}\fi}%%%%<<<---- here
\xydef@\xyPDFfillcirc@Special#1#2{%
 \ifx#2\relax\PDFmacro@{#1 sfc}%%%%%<<<---- here
 \else\PDFmacro@{#1 fc}\fi}%%%%<<<---- here
\xydef@\xyPDFfillellipse@Special#1#2{%
 \ifx#2\relax\PDFmacro@{#1 sfe}%%%%%<<<---- here
 \else\PDFmacro@{#1 fe}\fi}%%%%<<<---- here
\endinput


==> xypdf-l.tex <==
%% xypdf-l.tex from $Id: xypdf-l.doc,v $
%%
%% Xy-pic ``Line extension'' PDF backend support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-lloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-lloaded\endcsname=\empty \xycatcodes
\expandafter\ifx\csname xypdf-sloaded\endcsname\empty\else
 \xyinputorelse@{xypdf-s}{\xyerror@{Could not load xypdf-s}{}}%
 \xycatcodes\fi
\xydef@\installPDFline@{\installPDFstyle@
 \installPDFlinestyles@ \installPDFpolylines@ }
\xydef@\UsePDFlines{\installPDFline@}
\xydef@\NoPDFlines{\UnloadLine@\relax}
\xydef@\xyPDFlineSpecial@#1{\xyPDFrawZ@{ #1 w}}
\xydef@\xyPDFcapSpecial@#1{\xyPDFrawZ@{ #1 J}}
\xydef@\xyPDFjoinSpecial@#1{\xyPDFrawZ@{ #1 j}}
\xydef@\xyPDFmiterSpecial@#1{\xyPDFrawZ@{ #1 M}}
\xydef@\installPDFlinestyles@{%
 \let\xylinewidth@@=\xylinewidth@
 \let\transxyline@@=\transxyline@
 \let\xylineSpecial@@=\xyPDFlineSpecial@
 \let\resetxyline@@=\resetxyline@i
 \let\xy@linecap@@=\xy@linecap@
 \let\xycapSpecial@@=\xyPDFcapSpecial@
 \let\resetxylinecap@@=\resetxylinecap@i
 \let\xy@linejoin@@=\xy@linejoin@
 \let\xyjoinSpecial@@=\xyPDFjoinSpecial@
 \let\resetxylinejoin@@=\resetxylinejoin@i
 \let\xy@linemiter@@=\xy@linemiter@
 \let\xymiterSpecial@@=\xyPDFmiterSpecial@
 \let\resetxylinemiter@@=\resetxylinemiter@i
}
\xydef@\xypolylinePDF@Special#1{\PDFspecial@@{ q [] 0 d #1 S Q}}
\xydef@\xypolydotPDF@Special#1{\PDFspecial@@{ q [1 3] 0 d S Q}}
\xydef@\xypolydashPDF@Special#1{\PDFspecial@@{ q [5] 0 d #1 S Q}}
\xydef@\xypolyfillPDF@Special#1{\PDFspecial@@{ q #1 f Q}}
\xydef@\xypolyeofillPDF@Special#1{\PDFmacro@{ q #1 f* Q}}
\xydef@\installPDFpolylines@{%
 \let\xypolyline@Special=\xypolylinePDF@Special
 \let\xypolydot@Special=\xypolydotPDF@Special
 \let\xypolydash@Special=\xypolydashPDF@Special
 \let\xypolyfill@Special=\xypolyfillPDF@Special
%\let\xypolyeofill@Special=\xypolyeofillPDF@Special
 \let\xy@polystyle@@=\xy@polystyle@ }
\endinput


==> xypdf-r.tex <==
%% xypdf-r.tex from $Id: xypdf-r.doc,v $
%%
%% Xy-pic ``PDF Rotations and Scaling''.
%% Copyright (c) 1999-1999 Ross Moore <ross@maths.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-rloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-rloaded\endcsname=\empty \xycatcodes
\expandafter\ifx\csname xypdf-sloaded\endcsname\empty\else
 \xyinputorelse@{xypdf-s}{\xyerror@{Could not load xypdf-s}{}}%
 \xycatcodes\fi
\xydef@\installPDFrotscale@{\installPDFstyle@
% \let\xyRotate@@=\xyPDFrotate@@
% \let\doSpecialRotate@@=\doPDFspecialRotate@@
 \let\xyscale@@=\xyPDFscale@@
 \xyPDFshapes@true
 \xyuncatcodes }
\xydef@\UsePDFrotate{\installPDFrotscale@}
\xydef@\NoPDFrotate{\UnloadRotate@\relax}
\xydef@\xyPDFpretransform@{\xyPDFrawA@{\preXYtransform@@}}
\xydef@\xyPDFposttransform@{\xyPDFrawZ@{\postXYtransform@@}}
\let\preXYtransform@=\xyPDFpretransform@
\let\postXYtransform@=\xyPDFposttransform@
\xydef@\xyPDFrotSplit@{%
 \expandafter\def\expandafter\preShape@@\expandafter{\xyPDFpre@}%
 \expandafter\def\expandafter\postShape@@\expandafter{\xyPDFpost@}}
\xydef@\xyPDFscale@@#1#2{%
 \xyPDFsplitPDF@{\xyscale@start(#1,#2)}{\xyscale@end}%
 \xyPDFrotSplit@\xyPDFpdfxy@ }
\xydef@\xyPDFrotate@@#1{%
 \xyPDFsplitPDF@{\xyrot@start(#1 xyd)}{\xyrot@end}%%%<<------ here
 \xyPDFrotSplit@\xyPDFpdfxy@ }
\xydef@\xyPDFspecialRotate@#1{%
 \xyPDFsplitPDF@{\xyrot@start(#1)}{\xyrot@end}\xyPDFrotSplit@\xyPDFpdfxy@ }
\xydef@\doPDFspecialRotate@@#1@@{\xyPDFspecialRotate@{#1}}
\xydef@\xyRotScale@@{%
% \def\xyrot@start(##1){{xyt ##1\space xyr}}%%%<<------ here
 \def\xyscale@start(##1,##2){ q ##1 0 0 ##2 0 0 cm}%
 \def\xyrot@end{ Q}\def\xyscale@end{ Q}}
\endinput


==> xypdf-s.tex <==
%% xypdf-s.tex from $Id: xypdf-s.doc,v $
%%
%% Xy-pic ``Style extension'' PDF support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-sloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-sloaded\endcsname=\empty \xycatcodes
\xydef@\xykillstyles@@{\Unloadstyle@}%
\xywarnifdefined\xyPDFescapestyle@
\xywarnifdefined\xyPDFsplitescape@
{\xyuncatcodes \catcode`@=11
 \gdef\xyPDFescapestyle@#1@@{\xyPDFsplitescape@#1<><>@@}%
 \gdef\xyPDFsplitescape@#1<>#2<>#3@@{\xyescape@@{#1}{#2}}}
\xydef@\xyPDFsplitPDF@#1#2{%
 \def\xyPDFpre@{#1}\def\xyPDFpost@{#2}\modPDFboxz@ }
\xydef@\xyescape@@#1#2{\checkXyStyle@ 
 \applyFIFOstyle@\prexyescape@{#1}\postxyescape@{#2}}
\xydef@\prexyescape@{\xyescapeSpecial@}
\xydef@\postxyescape@{\xyescapeSpecial@}
\xylet@\xyescapeSpecial@=\eat@
\let\xyescapeSpecial@=\addtostyletoks@
\xydef@\installPDFstyle@{%
 \def\preXYstyle@@{\xyPDFpre@}%
 \let\xydoprestyles@=\xyPDFrawstyleA@
 \let\xydopoststyles@=\xyPDFrawZ@
 \let\xykillstyles@=\xykillstyles@@
 }
\xydef@\xyPDFrawstyleA@#1{\xyPDFrawA@{{#1}{}}}
\endinput


==> xypdfpdf.tex <==
%% xypdfpdf.tex from $Id: xypdfpdf.doc,v $
%%
%% Xy-pic ``PDF-PDF'' PDF support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@ens-lyon.fr>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-pdfloaded\endcsname=\empty \xycatcodes
\global\newif\ifPDFspecials@
\xylet@\PDFmacro@@=\eat@
\xylet@\PDFdict@@=\eat@
\xylet@\PDFspecial@@=\eat@
\xylet@\PDFread@@=\eat@
\xylet@\PDFinclude@@=\eat@
\xylet@\PDFraw@@=\eat@
\xylet@\xyPDFobeylines@@=\relax
\xylet@\PDFspecialdict@@=\eat@
\xydef@\UnloadPDFpdf@{%
 \let\PDFmacro@@=\eat@
 \let\PDFdict@@=\eat@
 \let\PDFspecial@@=\eat@
 \let\PDFread@@=\eat@
 \let\PDFinclude@@=\eat@
 \let\PDFraw@@=\eat@
 \let\xyPDFobeylines@@=\relax
 \let\PDFspecialdict@@=\eat@
}
\xydef@\UnloadPDF@{\UnloadPDFpdf@
 \expandafter\ifx\csname xypdfloaded\endcsname\unknown\PDFspecials@false
 \else\expandafter\NoPDFspecials\fi}
\xylet@\UnloadPDF@@=\UnloadPDF@
\ifx\undefined\dvitype@\xydef@\dvitype@{null}\fi
\xylet@\xyrealshipout@=\shipout
\xydef@\xyPDFshipout@{\xyrealshipout@}
\xydef@\firstPDF@{%
 \global\let\firstPDF@@=\relax \global\let\firstPDF@=\relax}
\xylet@\firstPDF@@=\firstPDF@
\xylet@\dumpPDFdict@@=\relax
\xydef@\installxypdf@{%
 \xyinputorelse@{xypdfpdf}{\xydrivernoload@{pdfpdf}}\xycatcodes
 \installxypdf@@ \installxypdf@x }
\xylet@\installxypdf@@=\relax
\xylet@\setupxyPDF@@=\PDFspecials@true
\xywithoption{pdf}{\let\setupxyPDF@@=\setupxyPDF@}
\xydef@\installxypdf@x{
 \let\firstPDF@=\relax
 \let\XYpredict@=\relax
 \setupxyPDF@@ }
\xydef@\setupxyPDF@{\PDFspecials@true}
\let\realinstallxypdf@x=\installxypdf@x
\ifx\undefined\AfterBeginDocument
 \def\installxypdf@x{\xysetup@@{\realinstallxypdf@x}}%
\else
 \def\installxypdf@x{\AfterBeginDocument{\realinstallxypdf@x}}%
\fi
\xydef@\xydefaultdriver@{dvipdf}
\xydef@\xyPDFdriver#1{\def\xydefaultdriver@{#1}}
\xydef@\installxypdf@orig{\DN@{}%
 \ifx\xydriversselected@@\empty
 \DN@{\expandafter\defaultinstallpdf@\expandafter{\xydefaultdriver@}}%
 \else \def\do##1{%
 \expandafter\ifx\csname##1@xy@pdf\endcsname\relax
 \DN@{\defaultinstallpdf@{##1}}}%
 \xydriversselected@@ 
 \else \DN@##1{}\fi\fi \next@ }
\xydef@\defaultinstallpdf@#1#2{%
 \xywarning@{no driver specified, using #1 }%
 \xyrequire{#1}\csname #1@xy@pdf\endcsname{}}
\xydef@\null@xy@pdf{\installxypdf@}
\xydefcsname@{shape [!...]}#1{%
 \expandafter\ifx\csname xypdf-sloaded\endcsname\empty \DN@{\xyPDFescapestyle@{#1}@@}%
 \else\ifxyPDFshapes@\DN@{\xyPDFshapechar@{#1}@@}%
 \else \DN@{\xyPDFcharwarning@}\fi\fi \next@ }
\xydefcsname@{shape [pdfxy]}{\ifxyPDFshapes@\DN@{\xyPDFpdfxy@}%
 \else \DN@{\xyPDFcharwarning@}\fi \next@ }
\xydef@\xyPDFpdfxy@{%
 \setboxz@h{\dimen@=\L@p \advance\dimen@-\R@p 
 \dimen@ii=-\U@p \raise\dimen@ii\hbox to\z@{%
 \kern\dimen@\xyPDFcurrpt@\kern-\dimen@}\boxz@}}%
\xydef@\xyPDFcurrpt@{\ifxyPDFshapes@\expandafter\xyPDFcurrpt@@\fi}
\xydef@\xyPDFcurrpt@@@{\PDFspecial@@{xyi}\PDFraw@@{userdict begin xyx end}}%%%%<<<<<--- here
\ifx\undefined\xyPDFcurrpt@@ \xylet@\xyPDFcurrpt@@=\xyPDFcurrpt@@@ \fi
\xywarnifdefined\xyPDFshapechar@
\xywarnifdefined\xyPDFsplitshape@
{\xyuncatcodes \catcode`@=11
 \gdef\xyPDFshapechar@#1@@{\xyPDFsplitshape@#1<><>@@}%
 \gdef\xyPDFsplitshape@#1<>#2<>#3@@{\xyPDFsplitPDF@{#1}{#2}}}
\xydef@\xyPDFrawA@#1{\expandafter\xyPDFrawAA@ #1{}{}}%
\xydef@\xyPDFrawAA@#1#2{\PDFraw@@{ #1 #2}\PDFmessage{ #1 #2 }}%
\xydef@\xyPDFrawZ@#1{\PDFraw@@{ #1}\PDFmessage{ #1 }}%
\xydef@\modPDFboxz@{%
 \expandafter\DN@\expandafter{\xyPDFpre@{}}\ifx\next@\empty\else
 \setboxz@h{\expandafter\xyPDFrawA@\expandafter{\xyPDFpre@{}}\boxz@
 \expandafter\xyPDFrawZ@\expandafter{\xyPDFpost@}}\DN@{}\fi}%
\xydef@\modPDFdrop@{%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawA@\expandafter{\xyPDFpre@{}}}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{\nextii@ ##1}}%
 \expandafter\next@\expandafter{\Drop@@}%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawZ@\expandafter{\xyPDFpost@}}%
 \DN@##1{\expandafter\def\expandafter\Drop@@\expandafter{\tmp@ ##1}}%
 \expandafter\next@\expandafter{\nextii@}}%
\xydef@\modPDFconnect@{%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawA@\expandafter{\xyPDFpre@{}}}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{\nextii@ ##1}}%
 \expandafter\next@\expandafter{\Connect@@}%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawZ@\expandafter{\xyPDFpost@}}%
 \DN@##1{\expandafter\def\expandafter\Connect@@\expandafter{\tmp@ ##1}}%
 \expandafter\next@\expandafter{\nextii@}}%
\xydef@\xyPDFpre@{{}{}}
\xydef@\xyPDFpost@{}
\xydef@\PDFmessage@#1{\W@{PDF: #1}}
\xydef@\PDFignore@#1{}%
\xydef@\showPDFmessages{\let\PDFmessage=\PDFmessage@}
\xydef@\hidePDFmessages{\let\PDFmessage=\PDFignore@}
\xylet@\PDFtracing=\showPDFmessages
\hidePDFmessages
\xydef@\PDFmacro@#1{\PDFmacro@@{#1}\PDFmessage{#1}}
\xydef@\includeXYPDFdict@{\relax}
\xydef@\xyPDFdictknown@{}
\xywarnifdefined\obeyoutlines@
{\catcode`\^^M=\active%
 \gdef\obeyoutlines@{\catcode`\^^M=\active \def^^M{^^J}%
 \newlinechar=`\^^J\obeyspaces}}
\xynew@{if}\ifxyPDFshapes@ \xyPDFshapes@true 
\xydef@\xyPDFcharwarning@@{\xyPDFcharmessage@
 \gdef\xyPDFcharwarning@@{\xyPDFcharmessage@
 \xywarning@{...no further PDF warnings will be given}%
 \global\let\xyPDFcharwarning@@=\relax }}
\xydef@\xyPDFcharmessage@{\xywarning@{%
 the current <driver> does not fully support PDF effects}}%
\xydef@\newxyshape#1#2#3{%
 \DN@{#3}\ifx\next@\empty
 \xydefcsname@{shape [#1]}{\csname xyshape@#1@\endcsname}%
 \else \expandafter\def\csname shape [#1]\endcsname{%
 \csname xyshape@#1@\endcsname}\fi
 \DN@{#2}\ifx\next@\empty
 \expandafter\def\csname xyshape@#1@\endcsname{%
 \xyundefinedEffect@{#1}{}@@}%
 \else \expandafter\def\csname xyshape@#1@\endcsname{#2}\fi }
\xydef@\xyundefinedEffect@#1#2@@{%
 \xywarning@{The #1 #2 effect is not implemented with the current driver}}%
\xydef@\newxyPDFshape#1#2{%
 \expandafter\DN@\expandafter{\csname shape [#1]\endcsname}%
 \DNii@{\relax}\ifx\next@\nextii@ \newxyshape{#1}{}\relax\fi
 \expandafter\DNii@\expandafter{\csname xyPDFshape@#1@\endcsname}%
 \expandafter\def\nextii@{#2}%
 \ifx\nextii@\empty\expandafter\def\next@{\xyPDFnotimplemented@@`#1'@@}%
 \else
 \edef\tmp@{\noexpand\let\expandafter\noexpand\next@
 \expandafter\noexpand\nextii@}%
 \expandafter\tmp@\fi }
\xydef@\xyPDFnotimplemented@@#1@@{%
 \xywarning@{This PostScript effect is not implemented yet}}%
\xydef@\xyPDFnotfinished@@{%
 \xywarning@{This effect is not reliable yet; box sizes may be wrong}}%
\installxypdf@
\endinput








==> xypdftex.tex <==
%% xypdftex.tex from $Id: xypdftex.doc,v $
%%
%% Xy-pic ``pdf-TeX'' driver interface option.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{pdftex}{pdf-TeX driver}{\stripRCS$Revision: 3.8 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\pdfTeX@@#1{\dvimessage@{pdf-TeX}{#1}}
\newdriver{%
 \xyaddsupport{color}\pdftexColor@@
 \xyaddsupport{crayon}\pdftexCrayon@@
% \xyaddsupport{pdf}\pdftexPDF@@
% \xyaddsupport{rotate}\pdftexRotate@@
 \xyaddsupport{line}\pdftexLine@@
% \xyaddsupport{frame}\pdftexFrames@@
% \xyaddsupport{tile}\pdftexTiles@@
 \xyaddsupport{cmtip}\relax
}
%\xydef@\pdfTeXcolor@push#1{\special{pdfcolor push}\special{pdfcolor #1}}
\xydef@\pdfTeXcolor@push#1{\edef\pdfsaved@color{\pdfcurrent@color}%
 \def\pdfcurrent@color{#1}\special{#1}}%%%<<<<<<--- WRONG !
\xydef@\pdfTeXcolor@pop{\let\pdfcurrent@color\pdfsaved@color
 \expandafter\special\expandafter{\pdfsaved@color}}
\xydef@\pdfTeXcolours@{\pdftexPDFtypes@
% \let\xylocalColor@=\xystackcolor@
% \let\xycolor@push=\pdfTeXcolor@push
% \let\xycolor@pop=\pdfTeXcolor@pop
 \def\xycolor@{\xycolor@@}%
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-c}{\xydrivernoload@{pdf-c}}%
 \if@pdf@known\installPDFcolor@ }\else\DN@{}\fi \next@
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\pdftexCrayon@@{}}%
 \else\let\next@=\xystandardcolors@ \fi \next@ 
 \let\xycolorwarning@=\relax \pdfTeX@@{color}%
 \let\pdftexColor@@=\relax
 \let\UnloadColor@@=\NopdfTeXcolor@
 }
\xydef@\pdftexColor@@{\pdfTeXcolours@}
\xydef@\NopdfTeXcolor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\pdftexColor@@=\pdfTeXcolours@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\pdftexCrayon@@{\pdftexColor@@\pdftexCrayon@}
\xydef@\pdftexCrayon@{\installCrayolaColors@}%
\xydef@\pdftexPDF@@{\if@pdf@known\pdftexPDF@}
\xydef@\pdftexPDFunload@{\if@pdf@known\UnloadPDF@
 \let\UnloadPDF@@=\UnloadPDF@
 \let\pdftexPDF@@=\pdftexPDF@ }
\xydef@\pdftexPDFtypes@{%
 \xyinputorelse@{xypdfpdf}{\xydrivernoload@{pdfpdf}}%
 \ifx\PDFspecial@@\pdfTeXspecial@\else
 \let\PDFspecial@@=\pdfTeXspecial@
 \let\PDFmacro@@=\pdfTeXmacro@
 \let\PDFdict@@=\pdfTeXdict@
 \let\PDFraw@@=\pdfTeXraw@
 \let\PDFinclude@@=\pdfTeXinclude@
 \let\PDFspecialdict@@=\pdfTeXspecialDict@
 \let\xyPDFobeylines@@=\obeypdfTeXlines@
 \pdfTeX@@{PDF}%
 \fi \pdftexCurrpt@ }
\xydef@\pdfTeXspecial@#1{\if@pdf@known\firstPDF@@\pdfobj{#1}\pdflastobj}
\xydef@\pdfTeXmacro@#1{\pdfobj{#1}}
\xydef@\pdfTeXdict@#1{\pdfnames{#1}}
\xydef@\pdfTeXspecialDict@#1{\pdfnames{#1}}
\xydef@\pdfTeXinclude@#1{\if@pdf@known\firstPDF@@\special{prePDFfile #1}}
\xydef@\pdfTeXraw@#1{\if@pdf@known\firstPDF@@\pdfliteral{#1}}%
{\catcode`\^^M=\active%
 \gdef\next{\catcode`\^^M=\active \let^^M=\par%
 \let\PDFspecial@@=\pdfTeXdict@ \obeyspaces}}
\xylet@\obeypdfTeXlines@=\next
\xydef@\pdftexCurrpt@{\let\xyPDFcurrpt@@=\pdftexCurrpt@@}%
\xydef@\pdftexCurrpt@@{\PDFspecial@@{xyi}\PDFraw@@{userdict begin xyx end}}%%%%%<<<<<--- here
\xydef@\pdftexPDF@{\pdftexPDFtypes@
 \let\pdftexPDF@@=\relax
 \let\UnloadPDF@@=\pdftexPDFunload@ 
 \let\installxypdf@@=\relax \if@pdf@known\installxypdf@ }
\xydef@\pdftexRotate@@{\pdftexRotate@}
\xydef@\pdftexRotate@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-r}{\xydrivernoload@{pdf-r}}%
 \xyRotScale@@ \if@pdf@known\installPDFrotscale@ }%
 \else\DN@{\xydriverfail@{rotations are}\if@pdf@known\UnloadRotate@\relax}\fi
 \next@}
\xydef@\pdftexLine@@{\pdftexLine@}
\xydef@\pdftexLine@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-l}{\xydrivernoload@{pdf-l}}%
 \if@pdf@known\installPDFline@ }%
 \else\DN@{\xydriverfail@{line-widths are}\if@pdf@known\UnloadLine@\relax}\fi
 \next@ }
\xydef@\pdftexFrames@@{\pdftexFrames@}
\xydef@\pdftexFrames@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-f}{\xydrivernoload@{pdf-f}}%
 \if@pdf@known\installPDFframes@ }%
 \else\DN@{\xydriverfail@{frames are}\if@pdf@known\UnloadPDFframes@\relax}\fi
 \next@ }
\xydef@\pdftexTiles@@{\pdftexTiles@}
\xydef@\pdftexTiles@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-t}{\xydrivernoload@{pdf-t}}%
 \if@pdf@known\installPDFpatterns@ \xystandardpatterns@}%
 \else\DN@{\xydriverfail@{Patterns are}\if@pdf@known\UnloadPDFpatterns@\relax}\fi
 \next@ }
\xydef@\if@pdf@known#1{\ifx\undefined#1\else\expandafter#1\fi}
\xyendinput



